Provably-Safe, Online System Identification

Precise manipulation tasks require accurate knowledge of payload inertial parameters. Unfortunately, identifying these parameters for unknown payloads while ensuring that the robotic system satisfies its input and state constraints while avoiding collisions with the environment remains a significant challenge. This paper presents an integrated framework that enables robotic manipulators to safely and automatically identify payload parameters while maintaining operational safety guarantees. The framework consists of two synergistic components: an online trajectory planning and control framework that generates provably-safe exciting trajectories for system identification that can be tracked while respecting robot constraints and avoiding obstacles and a robust system identification method that computes rigorous overapproximative bounds on end-effector inertial parameters assuming bounded sensor noise. Experimental validation on a robotic manipulator performing challenging tasks with various unknown payloads demonstrates the framework's effectiveness in establishing accurate parameter bounds while maintaining safety throughout the identification process. The code is available at our project webpage: https://roahmlab.github.io/OnlineSafeSysID/.

==> Sections/00_Symbols.tex <==
\section*{List of Symbols}
\subsection*{Colors}
\begin{itemize}
  \item obstacles: red
  \item something terrible (collision, exceed torque limits, fail): orange
  \item robot: grey-white
  \item groundtruth of inertial parameters / 0 and ultimate bound in the tracking error plot: black solid line
  \item results of our method, for example, tracking error plots: green solid line
  \item results of variants our method, for example, tracking error plots: different kinds of blue (selected from colorbrewer) solid line
  \item results of other robust/adaptive controllers: different kinds of purple (selected from colorbrewer), solid line
  \item results of gravity compensation PD controller: purple, solid line
\end{itemize}

\subsection*{General Symbols}
\begin{itemize}
  \item $[\ubar{x},\bar{x}]$: interval
  \item $f([\ubar{x},\bar{x}])$: function evaluation over an interval
  \item $[f]([\ubar{x},\bar{x}])$: function evaluation over an interval using interval arithmetic
  \item tr: trace of a matrix
  \item $V \in \N^+$: degree of Bezier curve.
  \item $v \in \{0, 1, \cdots, V\}$: index for Bernstein polynomials.
  \item $b_v \in \R$: $v$th Bezier coefficients.
  \item $P_v: [0, 1] \rightarrow \R$: $v$th Bernstein polynomials.
  \item $b: [0, 1] \in \R$: Bezier curve.
\end{itemize}

\subsection*{Robot Dynamics}
\begin{itemize}
  \item $T > 0$: some final time. Also length(duration) of a trajectory
  \item $t \in [0,T]$: some time
  % \item $I$: Identity matrix
  % \item $\textbb{0}$: Vector of zeros
  \item $n > 0$: number of joints in the robot
  \item $j \in {1, 2, \cdots, n}$: joint/link index
  \item $\Q \subset \R ^ n$: robot configuration space
  \item $q: [0, T] \rightarrow \Q$: robot joint trajectory
  \item $H$: inertia mass matrix.
  \item $C$: Coriolis matrix.
  \item $g$: gravity vector.
  \item $p$: system momentum.
  \item $\tau: [0, T] \rightarrow \R ^ n$: applied torque.
  \item $W$: inverse dynamics regressor.
  \item $W_p$: passivity-based inverse dynamics regressor.
  \item $W_m$: momentum regressor.
  \item $W_c$: indirect regressor that helps compute the time-derivative of momentum.
  \item $\theta_{\text{ip}, j} \in \R ^ {10}$: inertial parameter of $j$th link.
  \item $\theta_{\text{f}, j} \in \R ^ 4$: friction parameter of $j$th joint.
  \item $\theta_{\text{ip}} \in \R ^ {10n}$: inertial parameter of all links.
  \item $\theta_{\text{f}} \in \R ^ {4n}$: friction parameter of all joints.
  \item $\theta \in \R ^ {14n}$: dynamical parameters of the whole robot.
  \item $\theta_{e} \in \R ^ {10}$: inertial parameters of the end effector.
  \item $\theta_0$: nominal dynamical parameters.
  \item $[\theta]$: overapproximated interval for dynamical parameters.
  \item $\nomparamsend$: nominal dynamical parameters of end effector.
  \item $\intparamsend$: overapproximated interval for dynamical parameters of the robot excluding the end effector.
  \item $\nomparamsrobot$: nominal dynamical parameters of end effector.
  \item $\intparamsrobot$: overapproximated interval for dynamical parameters of the robot excluding the end effector.
  \item $I_j$: shifted inertia tensor of $j$th link.
  \item $\text{LMI}(\inertialparamsj)$: LMI constraint for inertial parameters of $j$th link.
  \item $\eta$: Log-Chelosky parameterization of $\inertialparamsj$.
  \item $\eta_e$: Log-Chelosky parameterization of the end effector inertial parameters.
  \item $P: \R^{10} \rightarrow \R^{10}$: map from $\eta$ to $\inertialparamsj$.
  \item $M(\eta)$: Upper trianglar matrix decomposition of LMI matrix.
  \item $\alpha, d_1, d_2, d_3$: diagonal entries of Log-Chelosky matrix.
  \item $s_{21}, s_{31}, s_{32}, s_{41}, s_{42}, s_{43}$: upper triangular entries of Log-Chelosky matrix.
\end{itemize}

\subsection*{Controller}
\begin{itemize}
  \item $q_d: [0, T] \times \K \rightarrow \Q$: desired trajectory.
  \item $k \in \K \subset \R^{n_k}$: trajectory parameters.
  \item $\qA$: total feedback trajectory.
  \item $\dqm$: modified desired trajectory.
  \item $r$: error trajectory.
  \item $\unom$: nominal control input.
  \item $\urob$: robust feedback input.
  \item $w(\qA, \nomparams, \trueparams)$: disturbance.
  \item $[w(\qA, \nomparams, \intparams)]$: bound of disturbance.
  \item $\rho([w(\qA, \nomparams, \intparams)])$: measure of worst-case disturbance.
  \item $\lambdamin$: minimum eigenvalues of inertia mass matrix.
  \item $\lambdamax$: maximum eigenvalues of inertia mass matrix.
  \item $\sigmin$: lower bound of minimum eigenvalues of inertia mass matrix.
  \item $\sigmax$: upper bound of maximum eigenvalues of inertia mass matrix.
  \item $\varepsilon$: ultimate bound.
  \item $V_M$: upper bound of Lyapunov function
\end{itemize}

\subsection*{System Identification}
\begin{itemize}
  \item $\boldsymbol{q}_{1:N}$: collection of joint position measurements.
  \item $\boldsymbol{\dot{q}}_{1:N}$: collection of joint velocity measurements.
  \item $\boldsymbol{\tau}_{1:N}$: collection of applied torque measurements.
  \item $h \in \mathbb{N}^+$: forward integration horizon.
  \item $N_h \in \mathbb{N}^+$: number of forward integration horizons.
  \item $Y_{i:i+h}$: observation subregressor based on momentum.
  \item $U_{i:i+h}$: observation response subvector.
  \item $\boldsymbol{Y}(\boldsymbol{q}_{1:N}, \boldsymbol{\dot{q}}_{1:N})$: observation matrix based on momentum.
  \item $\boldsymbol{U}(\boldsymbol{q}_{1:N}, \boldsymbol{\dot{q}}_{1:N}, \boldsymbol{\tau}_{1:N}, \trueparamsrobot)$: observation response.
  \item $\eta_e^*$: optimal solution of system identification problem.
  \item $\meas$: collection of problem parameters: torque measurement and $\trueparamsrobot$.
  \item $\delta \meas$: collection of problem parameters: torque measurement and $\trueparamsrobot$.
  \item $[\delta \meas]$: collection of problem parameters: torque measurement and $\trueparamsrobot$.
  \item $D_{\eta_e \eta_e}$: gradient of the first-order optimality condition with respect to $\eta_e$.
  \item $D_{\eta_e \meas}$: gradient of the first-order optimality condition with respect to $\meas$.
  \item $\boldsymbol{W}(\boldsymbol{q}_{1:N}, \boldsymbol{\dot{q}}_{1:N}, \boldsymbol{\ddot{q}}_{1:N})$: observation matrix based on inverse dynamics.
\end{itemize}
